Speech Tokenizer is Key to Consistent Representation

Speech tokenization is crucial in digital speech processing, converting continuous speech signals into discrete units for various computational tasks. This paper introduces a novel speech tokenizer with broad applicability across downstream tasks. While recent advances in residual vector quantization (RVQ) have incorporated semantic elements, they often neglect critical acoustic features. We propose an advanced approach that simultaneously encodes both linguistic and acoustic information, preserving prosodic and emotional content. Our method significantly enhances speech representation fidelity across diverse applications. Empirical evaluations demonstrate its effectiveness in speech coding, voice conversion, emotion recognition, and multimodal language modeling, without requiring additional training. This versatility underscores its potential as a key tool for advancing AI-driven speech processing.

==> tmp.tex <==
% ----------------------------------------
% % Audio tokenize를 효율적으로 design하기 위해 semantic and acoustic feature를 함께 고려한다. Semantic information을 고려하기 위해 encoding된 embedding vector를 HuBERT~\cite{Hsu2021}를 teacher model로 같은 laten space로 embedding시키는 SpeechTokenizer~\cite{Zhang2024}방법을 사용한다. 
% %Prosody, pitch, timber와 같은 acoustic information을 고려하기 위해서는 Paralinguistic feature extraction을 teacher model로써 사용해 latent space에서 embedding시킨다. Paralinguistic feature extraction으로 ECAPA-TDNN을 사용하여 acoustic feature를 효율적으로 표현한다.
% % Audio Signal을 효과적으로 Quantization하기 위한 encoder는 Encodec model을 사용한다.~\cite{Défossez2022}
% In this study, we propose a method that simultaneously considers semantic and acoustic features for efficient audio tokenization. Specifically, to effectively utilize semantic information, we adopt the SpeechTokenizer approach~\cite{Zhang2024}, which maps encoded embedding vectors into the same latent space using HuBERT~\cite{Hsu2021} as a teacher model.
% To account for acoustic information such as prosody, pitch, and timbre, we employ paralinguistic feature extraction as a teacher model to embed these features in the latent space. Specifically, we utilize ECAPA-TDNN for paralinguistic feature extraction~\cite{Desplanques2020}, which efficiently represents acoustic features.
% For effective quantization of audio signals, we employ the EnCodec model as our encoder~\cite{Defossez2022, zeghidour2021}.
% The overall framework of the proposed method is illustrated in Figure~\ref{fig2_architecture:proposed_framework}.

% \subsection{Feature embedding}
% \label{ssec:subhead}
% % Audio Encoder에서 나온 entangled latent feature를 semantic and acoustic feature로 disentangle시키기 위해 각 feature를 효과적으로 extract시키는 모델을 사용한다. 본 section에서는 두 model을 통해 encoder에 나온 feature를 효과적을 disentangle 시키는 방법을 소개한다.
% To disentangle the entangled latent features generated by the audio encoder into semantic and acoustic features, we employ models that effectively extract each type of feature. In this section, we introduce the methods used to efficiently disentangle these features from the encoder output using the two proposed models.
% \subsubsection{Semantic feature}
% \label{sssec:subsubhead}
% % 우리는 semantic information을 효과적으로 뽑기위해 HuBERT를 사용하며 이것은 SpeechTokenzer에서 사용한 방식과 동일한 방식을 사용한다.
% % 학습에 사용하는 loss는 HuBERT를 teacher model로 두고 encoder를 나온 embedding feature에 distillation loss를 걸어서 학습한다. 이렇게 되면 encoder를 나온 embedding feature를 Quantization한 code값은 semantic information을 가지도록 학습되며 embedding feature와의 residual값은 semsntic information을 제외한 값의 residual값이 넘어게가 된다.
% We utilize HuBERT to effectively extract semantic information, employing the same approach as that used in the SpeechTokenizer. The loss function used for training involves leveraging HuBERT as the teacher model and applying distillation loss to the embedding features produced by the encoder. This approach ensures that the quantized code values derived from the encoder's embedding features capture semantic information, while the residual values represent components of the embedding features that are not associated with semantic information.
% \subsubsection{Acoustic feature}
% \label{sssec:subsubhead}
% % Acoustic feature를 뽑기위해 pretrained ECAPA-TDNN model을 가져와 사용한다. 이때 VQ를 통한 code vector와 dimension을 일치 시키기위해 align layer를 사용하며 이렇게 동작되는 과정을 Figure~\ref{fig:subfig1}에서 보여준다. VQ를 통해 나온 code값과, align layer를 통해 나온 feature값의 distribution을 같은 distribution상에 존재시키기 위해 Kullback-Leibler divergence loss를 사용해서 학습한다.
% To extract acoustic features, we utilize a pretrained ECAPA-TDNN model. An align layer is employed to match the dimensions of the code vectors obtained through vector quantization (VQ). The process of this alignment is illustrated in Figure~\ref{fig:subfig1}. To ensure that the distributions of the VQ code vectors and the features from the align layer converge, we incorporate a Kullback-Leibler divergence loss during training.
% \begin{equation}
% D_{KL}(P || Q) = \sum_{x} P(x) \log \frac{P(x)}{Q(x)}
% \label{eq:KL}
% \end{equation}
% In Equation (\ref{eq:KL}), p(x) represents the quantized code obtained by converting the input vector into a discrete codebook vector using the proposed vector quantization module, and Q(x) represents the continuous probability distribution generated by the alignment layer.
% % \begin{figure*}[t!]
% %     \centering
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{fig3_a.png}
% %         \caption{}
% %         \label{fig:subfig1}
% %     \end{subfigure}
% %     \hfill
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{fig3_b.png}
% %         \caption{}
% %         \label{fig:subfig2}
% %     \end{subfigure}
% %     \caption{(a) Acoustic feature extraction using the Align layer (b) Structure of the Align layer}
% %     \label{fig:combined_figure}
% % \end{figure*}
% ----------------------------------------
